Sampling real algebraic varieties for topological data analysis

Topological data analysis (TDA) provides a growing body of tools for computing geometric and topological information about spaces from a finite sample of points. We present a new adaptive algorithm for finding provably dense samples of points on real algebraic varieties given a set of defining polynomials. The algorithm utilizes methods from numerical algebraic geometry to give formal guarantees about the density of the sampling and it also employs geometric heuristics to reduce the size of the sample. As TDA methods consume significant computational resources that scale poorly in the number of sample points, our sampling minimization makes applying TDA methods more feasible. We provide a software package that implements the algorithm and also demonstrate the implementation with several examples.

==> arxiv v2/macros.tex <==
\usepackage{url}
\usepackage{amsmath}
\usepackage{array}
\usepackage{amsfonts}
\usepackage{enumerate}
\usepackage{graphicx}
\usepackage{wrapfig} 
\usepackage{xcolor} 
\usepackage{stmaryrd}
\usepackage{tipa}
\usepackage{float}
\usepackage{bbm} 
\usepackage{tikz}
\usepackage{algpseudocode}
\usepackage{algorithm}
\usepackage{mathtools}
\usepackage{afterpage}
\usepackage{pdflscape}
\usepackage{capt-of}
\usepackage{epstopdf}
\usepackage{setspace}
\usepackage{changepage}
\usepackage{tabularx}
\usepackage{geometry}
\usepackage{fancyhdr}
\usepackage{amssymb}
\usepackage{tikz-cd}
% Let top 85% of a page contain a figure
\renewcommand{\topfraction}{0.85}

% Default amount of minimum text on page (Set to 10%)
\renewcommand{\textfraction}{0.1}

% Only place figures by themselves if they take up more than 75% of the page
\renewcommand{\floatpagefraction}{0.75}

% Basic math operators that are probably the most universal to 
% all documents
\newcommand{\mz}{\mathbb{Z}}
\newcommand{\mr}{\mathbb{R}}
\newcommand{\mn}{\mathbb{N}}
\newcommand{\mq}{\mathbb{Q}}
\newcommand{\mc}{\mathbb{C}}
\newcommand{\del}{\partial}
\newcommand{\twid}{{\raise.17ex\hbox{$\scriptstyle\sim$}}}
\DeclareMathOperator{\im}{Im}
\DeclareMathOperator{\ext}{Ext}
\DeclareMathOperator{\Hom}{Hom}
\DeclareMathOperator{\coker}{coker}
\newcommand{\id}{\mathbbm{1}}
\newcommand{\si}{\mathcal{I}}

% Homological algebra 
\newcommand{\ilim}{\varprojlim}
\newcommand{\limone}{\varprojlim^1\nolimits}
\newcommand{\dlim}{\varinjlim}
\newcommand{\mzp}{\mz_{p^\infty}}  % The limit of Z/p -> Z/p^2 -> ...

% Covering spaces
\newcommand{\xtil}{\tilde{X}}
\newcommand{\lxtil}{\tilde{x}}
\newcommand{\inv}{^{-1}}
\newcommand{\btil}{\tilde{b}}
\newcommand{\ltil}{\tilde{\ell}}

% Category theory 
\newcommand{\mcalc}{\mathcal{C}}
\newcommand{\cop}{\mathcal{C}^{\text{op}}}
\newcommand{\bset}{\textbf{Set }}
\newcommand{\bpos}{\textbf{Pos }}
\newcommand{\crel}{\textbf{CRel }}
\newcommand{\lbrac}{\llbracket}
\newcommand{\rbrac}{\rrbracket}
\newcommand{\pfin}{\mathbf{P_{fin}}}
\newcommand{\upv}{\Lambda}
\newcommand{\app}{\text{App}}
\newcommand{\alar}[1]{\xrightarrow{\alpha_{#1}}}
\newcommand{\arr}[1]{\xrightarrow{#1}}
\newcommand{\al}[1]{\xleftarrow{#1}}
\newcommand{\all}[1]{\xleftarrow{\alpha_{#1}}}


% Machine Learning
\newcommand{\xbold}{\mathbf{x}}
\newcommand{\xibold}{\mathbf{x}_i}
\newcommand{\ybold}{\mathbf{y}}
\newcommand{\mubold}{\mathbf{\mu}}
\newcommand{\xtrans}{\xbold^{\mathbf{T}}}
\newcommand{\wbold}{\mathbf{w}}
\newcommand{\wsub}{w_0}
\newcommand{\iprob}{p^{a_i}_{b_i,c_i}}
\newcommand{\simb}{M_{a_i,b_i}}
\newcommand{\simc}{M_{a_i,c_i}}
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator{\sgn}{sgn}
\DeclareMathOperator{\softmax}{softmax}


% TDA 
\DeclareMathOperator{\pix}{pix}
\DeclareMathOperator{\mult}{mult}
\DeclareMathOperator{\topo}{\textbf{Top}}
\DeclareMathOperator{\pair}{\textbf{Pair}}
\DeclareMathOperator{\fdv}{\textbf{FDVec}}
\DeclareMathOperator{\hfs}{hfs}

% Algebraic geometry
\DeclareMathOperator{\mv}{\mathcal{V}}
\DeclareMathOperator{\mvr}{V_\mr}



% Thesis
\DeclareMathOperator{\minp}{\textsc{MinPoint}}
\DeclareMathOperator{\critp}{\textsc{CritPoint}}
\DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}
\DeclarePairedDelimiter{\floor}{\lfloor}{\rfloor}

